Out-of-distribution Few-shot Learning For Edge Devices without Model Fine-tuning

Few-shot learning (FSL) via customization of a deep learning network with limited data has emerged as a promising technique to achieve personalized user experiences on edge devices. However, existing FSL methods primarily assume independent and identically distributed (IID) data and utilize either computational backpropagation updates for each task or a common model with task-specific prototypes. Unfortunately, the former solution is infeasible for edge devices that lack on-device backpropagation capabilities, while the latter often struggles with limited generalization ability, especially for out-of-distribution (OOD) data. This paper proposes a lightweight, plug-and-play FSL module called Task-aware Normalization (TANO) that enables efficient and task-aware adaptation of a deep neural network without backpropagation. TANO covers the properties of multiple user groups by coordinating the updates of several groups of the normalization statistics during meta-training and automatically identifies the appropriate normalization group for a downstream few-shot task. Consequently, TANO provides stable but task-specific estimations of the normalization statistics to close the distribution gaps and achieve efficient model adaptation. Results on both intra-domain and out-of-domain generalization experiments demonstrate that TANO outperforms recent methods in terms of accuracy, inference speed, and model size. Moreover, TANO achieves promising results on widely-used FSL benchmarks and data from real applications.

==> doc/theory.tex <==
\section{Theoretical Analysis}

Note that in Eqn.(\ref{bn_1}) and (\ref{bn_2}), if we treat the intermediate feature $z_{i,j,r}$ as a vector in $\mathbb{R}^{m}$ following~\cite{sun2019newnorm},
the running mean $\mu_{i,j,r}$ and the running variance $\sigma_{i,j,r}$  actually map $z_{i,j,r}$ to a $(m-2)$-dimension sphere $\mathbb{S}^{m-2}_{\sqrt{m}}(\boldsymbol{0})$ with radius $\sqrt{m}$ and center origin via the mapping $(z_{i,j,r}-{\mu}_{i,j,r})/\sigma_{i,j,r}$.
These two parameters represent the statistical approximation of data distribution. 
Moreover, the parameters $\gamma_{i,j,r}$ and $\beta_{i,j,r}$ further map the normalized $(z_{i,j,r}-{\mu}_{i,j,r})/\sigma_{i,j,r}$ to the sphere $\mathbb{S}^{m-2}_{\gamma_{i,r}\sqrt{m}}(\beta_{i,j,r})$, whose radius and center are determined by weight $\gamma_{i,j,r}$ and bias $\beta_{i,j,r}$, respectively.
In the training stage, ${\mu}_{i,j,r}$ and $\sigma_{i,j,r}$ are calculated from the batch data, while $\gamma_{i,j,r}$'s and $\beta_{i,j,r}$'s are learned such that all $z_{i,r}$'s could be mapped to the sphere $\mathbb{S}^{m-2}_{\gamma_{i,j,r}\sqrt{m}}(\beta_{i,j,r})$.
In the evaluation stage, the two parameters of the data distribution, i.e., $\mu_{i,j,r}$ and $\sigma_{i,j,r}$, are replaced by their moving averages in the training stage.
Together with the learned  $\gamma_{i,j,r}$ and $\beta_{i,j,r}$, these parameters aim to map the test vectors to the same sphere as that in training. If not, the prediction results would be untraceable (see Table~\ref{tab:singleDomain} for some evidence).
That may be because other network parameters except the normalization layers are learned to encode the inputs based on the specific normalization used in training.
Therefore, appropriate normalization statistics of data distribution play an important role in evaluation. 
Note that the above-mentioned parameters are domain-specific. Inputs from different domains lay on different spheres.
The TANO module provides a more appropriate normalization and thus achieves better accuracy.
In addition, with the TANO module, inputs from different domains tend to be normalized to a common sphere.
As a result, network parameters except for the BN layers would access more diverse samples with proper normalization compared with training a model assuming the data come from a single domain.

The intermediate feature in a deep neural network before a normalization layer can be treated as a vector in $\mathbb{R}^{m}$, which is mapped to a $(m-2)$-dimension sphere $\mathbb{S}^{m-2}{\sqrt{m}}(\boldsymbol{0})$ with radius $\sqrt{m}$ and center origin through the running mean $\mu{i,j,r}$ and the running variance $\sigma_{i,j,r}$ according to Eqn.(\ref{bn_1}) and (\ref{bn_2}). These two parameters serve as a statistical approximation of the data distribution, while the parameters $\gamma_{i,j,r}$ and $\beta_{i,j,r}$ further map the normalized $(z_{i,j,r}-{\mu}{i,j,r})/\sigma{i,j,r}$ to the sphere $\mathbb{S}^{m-2}{\gamma{i,r}\sqrt{m}}(\beta_{i,j,r})$, whose radius and center are determined by the learned weight $\gamma_{i,j,r}$ and bias $\beta_{i,j,r}$, respectively. In the training stage, ${\mu}{i,j,r}$ and $\sigma{i,j,r}$ are calculated from the batch data, while $\gamma_{i,j,r}$ and $\beta_{i,j,r}$ are learned so that all $z_{i,r}$'s could be mapped to the sphere $\mathbb{S}^{m-2}{\gamma{i,j,r}\sqrt{m}}(\beta_{i,j,r})$. In the evaluation stage, the moving averages of ${\mu}{i,j,r}$ and $\sigma{i,j,r}$ are used along with the learned $\gamma_{i,j,r}$ and $\beta_{i,j,r}$ to map the test vectors to the same sphere as that in training. The appropriate normalization statistics of data distribution play a crucial role in evaluation. The TANO module provides more appropriate normalization and helps inputs from different domains to be normalized to a common sphere. As a result, network parameters except for the BN layers can access more diverse samples with proper normalization, which improves the model's performance. It should be noted that the above-mentioned parameters are domain-specific, and inputs from different domains are mapped to different spheres.
